Vulnerabilities that arise from poor governance in Distributed Ledger Technologies

Distributed Ledger Technologies (DLTs) promise decentralization, transparency, and security, yet the reality often falls short due to fundamental governance flaws. Poorly designed governance frameworks leave these systems vulnerable to coercion, vote-buying, centralization of power, and malicious protocol exploits: threats that undermine the very principles of fairness and equity these technologies seek to uphold. This paper surveys the state of DLT governance, identifies critical vulnerabilities, and highlights the absence of universally accepted best practices for good governance. By bridging insights from cryptography, social choice theory, and e-voting systems, we not only present a comprehensive taxonomy of governance properties essential for safeguarding DLTs but also point to technical solutions that can deliver these properties in practice. This work underscores the urgent need for robust, transparent, and enforceable governance mechanisms. Ensuring good governance is not merely a technical necessity but a societal imperative to protect the public interest, maintain trust, and realize the transformative potential of DLTs for social good.

==> 1-intro.tex <==
Whilst some earlier work laid the foundations \cite{vishnumurthy2003karma}, \cite{dai1998b}, \cite{chaum1983blind}, \cite{back2002hashcash} it is the Bitcoin white paper \cite{nakamoto2008bitcoin} that is widely regarded to have kickstarted the Web 3 revolution. Satoshi Nakamoto proposes a peer-to-peer electronic cash system in the wake of the Great Recession of 2008. Blockchain was conceived as a reactionary and idealistic attempt to redistribute power and decentralise decision-making of financial service providers\footnote{Satoshi states in 2009: \emph{“The root problem with conventional currency is all the trust required to make it work. The central bank must be trusted not to debase the currency, but the history of fiat currencies is full of breaches of that trust. Banks must be trusted to hold our money and transfer it electronically, but they lend it in waves of credit bubbles with barely a fraction in reserve. We have to trust them with our privacy, trust them not to let identity thieves drain our accounts. Their massive overhead costs make micropayments impossible.”}\cite{Nakamoto2009}.}. 

Cryptocurrencies initially faced a shy uptake but exploded in value after 2017. At time of writing (November 2024), Bitcoin price is up by 24,801.30\% since it was created. Similarly, Ether increased by 1,985.73\%, Cardano by 929.34\% and Solana by 37,300\% \textcolor{red}{citation needed}. 
Cryptocurrencies are here to stay: governments have not only begun to regulate these assets (see: US regulation, Japan, Mica, etc), but also own and invest in them as well (el salvador, Brasil's Sovereign Strategic Bitcoin Reserve (RESBit), Argentina Opens Its Stock Market to Foreign Crypto ETF Opportunities), US, UK, Ukraine \url{https://www.coingecko.com/research/publications/government-bitcoin-holdings}. 

Although Satoshi Nakamoto conceived Bitcoin as a decentralised, peer-to-peer network, the reality is that it and many other cryptocurrencies are centralised, manipulable and can be undermined due to their governance protocols. Governance is critical to delivering the promise of decentralisation, and without good governance, the vulnerabilities that may arise are dire. These issues must be addressed to preserve the original purpose of using cryptocurrencies for social good. Cryptocurrencies have become a matter of public interest: they are used by governments (with defaulted economies), their combined market worth is of \$3.71 Trillion and the entry barrier to invest in them is very low, meaning many with low technical and financial literacy can and do participate and invest in these technologies. Whilst this is revolutionary, it is also highly dangerous: many victims have lost life's savings due to scams, hacks, heists and rug pulls without little to no compensation. Governance safeguards are necessary to ensure transparency, accountability and prevent monopolisation and theft of funds. 

Our work addresses the governance dimension of DLTs that is increasingly intersecting with public policy, regulation, and societal well-being. Cryptocurrencies and distributed ledger technologies (DLTs) are no longer niche financial tools; they are evolving into systems that challenge traditional governance models and require new frameworks for oversight, trust-building, and public protection. By identifying vulnerabilities and proposing governance best practices, this work contributes to the interdisciplinary dialogue on how digital technologies transform governance structures, impact public institutions, and necessitate regulatory adaptations. Ultimately, we hope this research informs policy-making, aids regulators in understanding systemic risks, and helps ensure that these technological innovations serve, rather than exploit, the public interest.











Governance is crucial to deliver the promise of decentralisation in DLTs, but not only that, it is critical to ensure security. Satoshi Nakamoto's white paper introduces Bitcoin: A Peer-to-Peer Electronic Cash System. Why? The motivation is clear: to avoid relying on a centralised financial institution. Explicitly, Satoshi states: \emph{As long as a majority of CPU power is controlled by nodes that are \textbf{not cooperating} to attack the network, they'll generate the longest chain and outpace attackers} \cite{nakamoto2008bitcoin}. The key security assumption made is that no cluster of nodes holds majority power in the network.
This work, amongst others \cite{vishnumurthy2003karma}, \cite{dai1998b}, \cite{chaum1983blind} spawned the Web3 revolution, that emerged in the aftermath of the Great Recession of 2008. 
Governments, central banks and financial institutions had lost credibility of the people as a consequence of their regulatory oversights, predatory lending and mixing of high-risk operations with low-risk ones \cite{chua2012us}, \cite{bordo2017central}, \cite{debrun2017strengthening}. 
In the United States alone, some of the consequences of the crisis included a fall in: the real GDP of \$650 billion (4.3\%)\cite{GDP}, net worth of household by \$11.5 trillion (17.3\%) \cite{households} and the number of employed people by 8.3 million \cite{employees}. Sub-prime mortgages and predatory lending practises disproportionally targeted racial minorities, \cite{masterson2019great}, \cite{kochhar2014wealth}, \cite{Sarra_Wade_2020} eroding the trust that citizens placed in their governing institutions to safe-guard their best interests \cite{van2017political}.
Aside from the dire financial effects, research has found that during or in the immediate aftermath of the recession, a number of countries experienced a shift in their government towards authoritarianism \cite{berg2015impact}.
DLTs offered an alternative: distributed trust, decentralised power, shared reward.

